AUTOSHAPE: An Autoencoder-Shapelet Approach for Time Series Clustering

Time series shapelets are discriminative subsequences that have been recently found effective for time series clustering (TSC). The shapelets are convenient for interpreting the clusters. Thus, the main challenge for TSC is to discover high-quality variable-length shapelets to discriminate different clusters. In this paper, we propose a novel autoencoder-shapelet approach (AUTOSHAPE), which is the first study to take the advantage of both autoencoder and shapelet for determining shapelets in an unsupervised manner. An autoencoder is specially designed to learn high-quality shapelets. More specifically, for guiding the latent representation learning, we employ the latest self-supervised loss to learn the unified embeddings for variable-length shapelet candidates (time series subsequences) of different variables, and propose the diversity loss to select the discriminating embeddings in the unified space. We introduce the reconstruction loss to recover shapelets in the original time series space for clustering. Finally, we adopt Davies Bouldin index (DBI) to inform AUTOSHAPE of the clustering performance during learning. We present extensive experiments on AUTOSHAPE. To evaluate the clustering performance on univariate time series (UTS), we compare AUTOSHAPE with 15 representative methods using UCR archive datasets. To study the performance of multivariate time series (MTS), we evaluate AUTOSHAPE on 30 UEA archive datasets with 5 competitive methods. The results validate that AUTOSHAPE is the best among all the methods compared. We interpret clusters with shapelets, and can obtain interesting intuitions about clusters in two UTS case studies and one MTS case study, respectively.

==> preliminaries.tex <==
% !TEX root = main.tex

\section{Preliminaries}\label{Preliminaries}
In this section, we present some preliminaries and problem statement.
We summarize the notations and their meanings in Table~\ref{table:summary of notations}.

\begin{table}[tbp]
\centering
\caption{Summary of frequently used notations}\label{table:summary of notations}
\resizebox{\linewidth}{!}{
  \begin{tabular}{c|l}
\hline
  Notation & Meaning \\
\hline
\hline
    $T$          & a univariate time series (\UTS) instance \\
                 & $T = (t_1,t_2,\cdots,t_i, \cdots,t_N)$,\\
                 & where $t_i$ is the $i$-th value in $T$ \\
                 & and $N$ is the length of $T$\\
\hline
  $D$            & a \UTS~dataset $(T_1,T_2, \cdots,T_M)$, \\
                 & where $M$ is the number of time series in $D$ \\
                 %& with the class label $C_m$, $_{1\le m\le M}$  \\
\hline
  $T_{a,b}$       & a subsequence $T_{a,b}$ of $T$, $(t_{a}, \cdots,t_{b})$, \\
                 & where $1 \le a \le b \le N$, \\
                 & $a$ and $b$, the beginning and ending positions \\
\hline
                 $\mathcal{C}$  & the label set \\
%\hline
%  $D_C$                 & $C$ is the label in $\mathcal{C}$; and  \\
%                 & for all $T \in D_C$, the label of $T$ is $C$\\
\hline
  $V$            & the number of variables/observations/dimensions \\
\hline
  $\mathbb{T}$   & a multivariate time series (\MTS) instance \\
                 & $\mathbb{T} = (T^1, T^2,\cdots,T^v\cdots, T^V)$, \\
                 & where $T^v = (t^v_1,t^v_2,\cdots,t^v_i, \cdots,t^v_N)$\\
\hline
  $\mathbb{D}$   & an \MTS\ dataset $(\mathbb{T}_1,\mathbb{T}_2, \cdots,\mathbb{T}_M)$, \\
                 & where $M$ is the number of \MTS\ in $\mathbb{D}$ \\
\hline
  $\mathcal{S}$  & the shapelet set \\
%\hline
%  $\tilde{\mathbb{T}}$   & \MTS\ after multivariate shapelet transformation \\
%\hline
%  $\tilde{\mathbb{D}}$   & \MTS\ dataset after multivariate shapelet transformation \\
\hline
          \end{tabular}
}
\end{table}

\begin{definition} \textbf{Univariate time series $T$}.\label{def:uts}
  A univariate time series (\UTS) instance $T$ is an ordered-value sequence
  $T = (t_1,t_2,\cdots,t_i, \cdots,t_N)$, where $N$ is the length of $T$, $t_i \in \mathbb{R}, i \in [1,\cdots,N]$. \qed
\end{definition}

\begin{definition} \textbf{Univariate time series dataset $D$.}\label{def:utsd}
  A univariate time series dataset $D$ is a set of \UTS~instances. $T_m$ is a time series.
  $C_{m}$ is the class label of $T_m$, where $C_m \in \mathcal{C}, {m \in [1,M]}$.
  $\mathcal{C} = \{0,1,2, \cdots,\mathcal{|C|}-1\}$, and $|\mathcal{C}|$
  denotes the number of classes. \qed
\end{definition}

\begin{definition} \textbf{Subsequence $T_{a,b}$}.
  Given a time series $T$, a subsequence $T_{a,b}$ of $T$ is $(t_{a}, \cdots,t_{b})$,
  where $1 \le a \le b \le N$, $a$ and $b$ are, respectively, the beginning and ending positions of the
  subsequence in $T$. \qed
\end{definition}

\begin{definition} \textbf{Distance between two time series}~\cite{fang2018efficient}.
    The distance of the sequence $T_p$ of the length $|T_p|$ and $T_q$ of the length $|T_q|$
    is denoted as (w.l.o.g.\ assuming $|T_q| \ge |T_p|$),
    \begin{multline}\label{equation:subsequence distance}
      {\dist(T_p,T_q)} = \\ \min\limits_{j=1, \cdots,|T_q|-|T_p|+1} \frac{1}{|T_p|}
      \sum_{l=1}^{|T_p|} {(tq_{j+l-1}-tp_{l})}^2,
    \end{multline}
    where $tq_i$ and $tp_i$ are the $i$-th value of $T_p$ and $T_q$, respectively. \qed
\end{definition}

Intuitively, $\dist$ calculates the distance of the shorter sequence $T_p$
to the most similar subsequence in $T_q$ (namely, best match location),
as shown in Figure~\ref{fig:sequence distance}.

\begin{figure}[tbp]
  \centering
  \subfigure[An illustration of the best match location of a subsequence $T_p$ in a time series $T_q$. The blue one is the best match location.]{
    \includegraphics[width=.24\textwidth]{fig/bestmatch.pdf}\label{fig:sequence distance}
  }
  \subfigure[An illustration of a multivariate time series dataset, extracted from Basicmotions, with $6$ variables, length $100$]{
    \includegraphics[width=.19\textwidth]{fig/basicmotion.pdf}\label{figure:MTS}
  }
  \caption{(a) The best match location;
    and (b) A \MTS\ dataset, Basicmotions~\cite{UEAArchive}}
\end{figure}

\begin{definition} \textbf{Unsupervised shapelet $S$}~\cite{zakaria2012clustering}.
  An unsupervised shapelet $S$ of the length $|S|$ is a time series subsequence,
  which represents a group of time series instances and discriminate it from other groups.
  That is, for all $T_j$ in this group, $\dist(T_j$, $S)$ is smaller than
  $\dist(T_k$, $S)$, where $T_k$ is time series in other groups. \qed
\end{definition}

\csgzli{It is natural to extend the definition of univariate time series and \UTS~dataset
  (Definition~\ref{def:uts} and Definition~\ref{def:utsd}) to multivariate time series.}

\begin{definition} \textbf{Multivariate time series $\mathbb{T}$}.
  A multivariate time series (\MTS) instance $\mathbb{T}$ is $(T^1, T^2,\cdots, T^V)$,
  where $V$ is the number of variables (a.k.a observations, dimensions) in $\mathbb{T}$.
  $T^v$ is an ordered-value sequence of length $N$, $T^v = (t^v_{1},t^v_{2}, \cdots,t^v_{N})$.
  For each specific timestamp $n \in [1,N]$, $t_n \in \mathbb{R}^{V}$
  consists of ${V}$ variables $\{t^1_{n}, t^2_{n},\cdots, t^V_{n}\}$. \qed
\end{definition}

\begin{definition} \textbf{Multivariate time series dataset $\mathbb{D}$}.
  A multivariate time series dataset $\mathbb{D}$ contains $M$ \MTS~instances.
  Denote the number of time series in $\mathbb{D}$ as $M$.
  $\mathbb{T}_m$ is a \MTS~instance with $C_m, {m \in [1,M]}$,
  where $C_{m} \in \mathcal{C}$ is the class label of the dataset,
  $\mathcal{C} = \{0,1,2, \cdots,\mathcal{|C|}-1\}$,
  and $|\mathcal{C}|$ denotes the number of classes. \qed
\end{definition}

The apparent difference between univariate and multivariate time series is that
there are multiple observations at each timestamp in \MTS.
An example of the \MTS~dataset, called Basicmotions from~\cite{UEAArchive},
is shown in Figure~\ref{figure:MTS}.
While the definition of shapelet can be naturally extended for \MTS,
the candidates of shapelet of \MTS~are voluminous,
which makes the clustering problem more difficult.

\begin{example}
  In Figure~\ref{figure:MTS}, six variables ($V = 6$) are recorded by an accelerometer and a gyroscope.
  In the dataset, there are four classes, \ie $|\mathcal{C}| = 4$,
  namely standing, walking, running, and playing badminton.
  Each class is accompanied with $10$ training cases (instances) and $10$ test cases.
  Thus, the overall number $M$ of instances is $80$.
  The length ($N$) of each time series is $100$.
  It is ineffective and inefficient to compute all the distances
  between each time series and numerous subsequences in the dataset. \qed
\end{example}

\noindent{\bf Problem statement}.
Given a multivariate time series dataset $\mathbb{D}$\footnote{An univariate time series dataset $D$ is a special case of an \MTS\ dataset $\mathbb{D}$.},
consisting of $M$ multivariate time series instances
$\mathbb{T}_1,\mathbb{T}_2,\cdots,\mathbb{T}_M$ with $V$ variables,
this paper investigates an unsupervised shapelet discovery method
for multivariate time series clustering. \qed

